Axiomatizations for downward XPath on Data Trees

We give sound and complete axiomatizations for XPath with data tests by "equality" or "inequality", and containing the single "child" axis. This data-aware logic predicts over data trees, which are tree-like structures whose every node contains a label from a finite alphabet and a data value from an infinite domain. The language allows us to compare data values of two nodes but cannot access the data values themselves (i.e. there is no comparison by constants). Our axioms are in the style of equational logic, extending the axiomatization of data-oblivious XPath, by B. ten Cate, T. Litak and M. Marx. We axiomatize the full logic with tests by "equality" and "inequality", and also a simpler fragment with "equality" tests only. Our axiomatizations apply both to node expressions and path expressions. The proof of completeness relies on a novel normal form theorem for XPath with data tests.

==> xp-semantics.tex <==
%!TEX root = main.tex
%
\newcommand{\emptystr}{\lambda} %notation for empty string
%
\begin{align*}
  \dbracket{\dow}^\Tt & = \{(x,y) \mid x \child y\} \\
%  \dbracket{\rtdow}^\Tt & = \textrm{reflexive transitive closure of }\dbracket{\dow}^\Tt\\
  \dbracket{\upw}^\Tt & = \{(x,y) \mid y \child x\} \\
%  \dbracket{\rtupw}^\Tt & = \textrm{reflexive transitive closure of }\dbracket{\upw}^\Tt\\
  \dbracket{\eps}^\Tt & = \{(x,x) \mid x \in T\}\\
  \dbracket{\alpha \beta}^\Tt & = \{(x,z) \mid (\exists y\in T)\ (x,y)
     \in \dbracket{\alpha}^\Tt,(y,z) \in \dbracket{\beta}^\Tt\} \\
  \dbracket{\alpha \cup \beta}^\Tt & = \dbracket{\alpha}^\Tt \cup \dbracket{\beta}^\Tt\\
  \dbracket{[\varphi]}^\Tt & = \{(x,x) \mid x \in \dbracket{\varphi}^\Tt\}\\
%
  \dbracket{a}^\Tt & = \{ x \in T  \mid \lbl(x) = a \}\\
  \dbracket{\lnot \varphi}^\Tt & =  T \setminus \dbracket{\varphi}^\Tt\\
  \dbracket{\varphi \land \psi}^\Tt & = \dbracket{\varphi}^\Tt \cap \dbracket{\psi}^\Tt\\
  \dbracket{\tup{\alpha}}^\Tt & = \{ x \in T \mid (\exists y\in T)\
     (x,y) \in \dbracket{\alpha}^\Tt \} \\
  \dbracket{\tup{\alpha = \beta}}^\Tt & = \{ x \in T \mid (\exists
    y,\!z\in T) (x,y) \in \dbracket{\alpha}^\Tt, (x,z) \in
  \dbracket{\beta}^\Tt, \data(y)=\data(z)\} \\
  \dbracket{\tup{\alpha \neq \beta}}^\Tt & = \{ x \in T \mid (\exists
    y,\!z\in T) (x,y) \in \dbracket{\alpha}^\Tt, (x,z) \in
  \dbracket{\beta}^\Tt, \data(y)\neq\data(z)\}
  \end{align*}

